REPA-G: Test-Time Conditioning with Representation-Aligned Visual Features

While representation alignment with self-supervised models has been shown to improve diffusion model training, its potential for enhancing inference-time conditioning remains largely unexplored. We introduce Representation-Aligned Guidance (REPA-G), a framework that leverages these aligned representations, with rich semantic properties, to enable test-time conditioning from features, in generation. By optimizing a similarity objective (the potential) at inference, we steer the denoising process toward a conditioned representation extracted from a pre-trained feature extractor. Our method provides versatile control at multiple levels of granularity, ranging from patch level matching via single patches to broad semantic guidance using global image feature tokens. We further extend this to multi-concept composition, allowing for the faithful combination of distinct concepts. REPA-G operates entirely at inference time with no additional training required, offering a flexible and precise alternative to often ambiguous text prompts or coarse class labels. Our approach achieves high-quality, diverse generations on ImageNet and COCO. Code is available at https://github.com/valeoai/REPA-G

==> fig/teasers/teaser_t2i_icml.tex <==
\begin{figure}[t]
    \centering
    \resizebox{\linewidth}{!}{
        \begin{tikzpicture}[
            column2/.style={anchor=center, font=\small, align=justify, text width=4.5cm},
            column3/.style={anchor=center},
            header/.style={font=\Large\bfseries, align=center, anchor=south},
            subhead/.style={font=\large\bfseries, text=black!90, anchor=north}, 
            rect/.style={fill=turquoise, draw=none, line width=0pt, draw opacity=0, minimum width=0.3cm, minimum height=0.3cm, inner sep=0pt}
        ]
            
            \draw[line width=1.pt, black!90] (-0.6, 0.45) -- (13.6, 0.45); 

            \draw[line width=1.pt, black!90] (-0.6,-0.4) -- (13.6,-0.4); 

            \draw[line width=1pt, black!90] (-0.6,-0.95) -- (6.5,-0.95); 
            \draw[line width=1pt, black!90] (6.8,-0.95) -- (13.6,-0.95); 

            \draw[black!90] (-0.6,-4.24) -- (6.7,-4.24);
            
            \draw[line width=1.pt, black!90] (-0.6,-7.5) -- (13.6,-7.5); 

            \draw[line width=1.pt, black!90] (6.7,-0.5) -- (6.7,-7.5);

            \node[header] at (3.05, -0.35) {Standard Conditionings};  %conditionings
            \node[header] at (10.25, -0.35) {\ours (ours)}; 

            \node[subhead] at (1.5, -0.4) {Condition};
            \node[subhead] at (4.9, -0.4) {Output};
            \node[subhead] at (8.5, -0.4) {Condition};    
            \node[subhead] at (12., -0.4) {Output}; 

            \node[column2, align=center] at (1.5, -2.6) {\textbf{Class Condition} \\ $\langle$Angora Rabbit$\rangle$};
            \node[column3] at (4.9, -2.6) {\includegraphics[width=3cm, height=3cm]{fig/teasers/rabbit_cls_cond.png}};
            \node[column3] at (12., -2.6) {\includegraphics[width=3cm, height=3cm]{fig/teasers/avg.png}};

            \node (orgim) at (8.1, -2.1) {\includegraphics[width=2.1cm, height=2.1cm]{fig/teasers/rabbit_org.png}};
            \node (volcano) at (8.1, -6.4) {\includegraphics[width=2.1cm, height=2.1cm]{fig/teasers/volcano.png}};
            \node (featmap) at (8.1, -3.7) {\includegraphics[width=0.8cm, height=0.8cm]{fig/teasers/rabbit_full_feat_map.png}}; 
            \node[left=-0.15cm of featmap, font=\scriptsize, align=center, rotate=90, anchor=south] {Image \\ Feats.};
            \node (targetfeat) at (8.1, -4.8) {\includegraphics[width=0.8cm, height=0.8cm]{fig/teasers/rabbit_feat.png}};
            \node[left=-0.15cm of targetfeat, font=\scriptsize, align=center, rotate=90, anchor=south] {Masked \\ Feats.};

            \draw[->, black, thick] (8.55,-3.7) -- (9.35, -3.7)
                node[midway, above, font=\scriptsize\bfseries] {Avg.}; 
            \node[rect, fill=orange] (dot2) at ([xshift=1.45cm,yshift=-0.0cm]featmap.center) {};
            \draw[->, black, thick] (9.75,-3.7) -- (10.45, -3.7)
                node[midway, above, font=\scriptsize\bfseries] {};
            \draw[->, black, thick] (8.55,-4.8) -- (10.45, -4.8)
                node[midway, above, font=\scriptsize\bfseries] {};

            \node[column2] at (1.5, -5.9) {
            \begin{minipage}{4cm}
                \centering \textbf{Text Prompt} \\ \smallskip
                \scriptsize A hyper-realistic, close-up of a fluffy white albino rabbit sitting on active volcanic terrain. Ground is cracked, blackened earth with fissures of bright, molten lava bubbling underneath. The light of lava casts an orange glow onto the rabbit's paws and lower fur. Rabbit has tall, upright ears. Background is dark, blurry volcanic landscape. High contrast, surreal, photorealistic.
            \end{minipage}
};
            \node[column3] at (4.9, -5.9) {\includegraphics[width=3cm, height=3cm]{fig/teasers/t2i_rabbit.png}};

            \node[rect] (dot) at ([xshift=1.45cm,yshift=-0.85cm]volcano.center) {};
            \draw[->,thick, black] (8.70, -7.26) -- (9.35, -7.26);

            \node[column3] at (12., -5.9) {\includegraphics[width=3cm, height=3cm]{fig/teasers/rabbit_on_fire.png}};
            \draw[->, black, thick] (9.75,-7.26) -- (10.45, -7.26)
                node[midway, above, font=\scriptsize\bfseries] {};


            \draw[
                draw=yellow,
                line width=1pt,
                opacity=1.0,    
                rounded corners=0pt
            ] 
            ($(volcano.north east) + (-0.55cm, -2.cm)$) 
            rectangle 
            ($(volcano.north east) + (-0.65cm, -2.1cm)$);

        \end{tikzpicture}
    }
    \caption{\textbf{Comparing class-label, text-prompt, and \ours conditioning.} All models are trained on ImageNet. \textit{(Top)} We average extracted features (\orangebox) from a anchor image to generate a generic ``rabbit'' image. \textit{(Bottom)} We combine a masked feature map with a specific ``lava'' patch (\turqoise) to synthesize a rabbit on a volcano. While text prompts require lengthy descriptions and often lack precision, our feature-based conditioning offers better compositional control and
    provides more precise generation.}
    \label{fig:teaser_cond_comparison}
\end{figure}


==> tab/coco_repa_cond/t2i.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Comparison with text-to-image (T2I) generation.} We compare our method against CAD-I \cite{cad}, an ImageNet-trained T2I baseline, using COCO validation captions as conditioning signals. Our method utilizes full and average feature maps extracted from REPA-E \cite{leng_repa-e_2025}. 
u}
\label{tab:t2i}
\renewcommand{\arraystretch}{1.2}
\resizebox{0.88\linewidth}{!}{%
\begin{tabular}{llccccc}
\toprule
\textbf{Model} &
\textbf{Cond.} &
\textbf{FID $\downarrow$} &
\textbf{sFID $\downarrow$} &
\textbf{IS $\uparrow$} &
\textbf{Prec. $\uparrow$} &
\textbf{Rec. $\uparrow$} \\
\midrule
CAD-I  & Text         & 37.98 & 29.87& 25.60 & 0.46 & 0.37 \\
REPA-E  & Avg. Feat.  & 3.58 & 11.10 & 32.69 & 0.75 & 0.78 \\
REPA-E & Full Feat.  & \textbf{2.11} & \textbf{8.35}  & \textbf{36.01} &  \textbf{0.98} & \textbf{0.96}\\
\bottomrule
\end{tabular}}
\end{table}



==> tab/multipot/multipot_scores.tex <==
\begin{table}[] % Change table to table* and use [t] for top alignment
\centering          % Centers the table on the page
\caption{\textbf{Compositional generation evaluation on ImageNet~\cite{deng2009imagenet}.} We assess visual quality with PickScore and concept adherence using CLIP, and compare \ours variants using IPA and SPA against standard baselines.}
\label{tab:multipot-metrics}
\resizebox{0.88\linewidth}{!}{%
\begin{tabular}{lccccc}
\toprule
\multirow{2}{*}{\textbf{Cond.}} & \textbf{Pick} & \textbf{CLIP} & \textbf{Target}& \textbf{Anchor} & \textbf{Combined} \\
& \textbf{Score} & \textbf{Score} & \textbf{Sim.}& \textbf{Sim.} & \textbf{Sim.} \\
\midrule
Uncond. & 0.175  & 0.100  & 0.098 & 0.113 & 0.105 \\ %
Class Cond. & \textbf{0.198 } & 0.220  & 0.110 & 0.243  & 0.177 \\ % Class Conditional
Interp. & 0.188 & 0.190  & 0.156  & 0.183 & 0.170 \\
\midrule
IPA\textrightarrow IPA & \uline{0.196 } & \uline{0.232} & \uline{0.372} & \textbf{0.452} & \uline{0.412} \\
IPA\textrightarrow SPA & \uline{0.196} & \textbf{0.238} & \textbf{0.510} & \uline{0.422 } & \textbf{0.466} \\
\bottomrule
\end{tabular}
}
\vspace{-3pt}
\end{table}



